Nagell-Lutz Theorem for Imaginary Quadratic Fields and class groups of quadratic fields

We prove the Nagell-Lutz theorem for the imaginary quadratic fields of class number one.

==> extra.tex <==
{\subsection{The family $y^2=x^3+(a+b\sqrt{-3})x$ over $\mathbb QQ(\sqrt{-3})$}

%Consider the elliptic curve 
$$E: y^2=x^3+(a+b\sqrt{-3})x$$
such that 
$$a^2+3b^2=p$$
here $p$ is a prime of the form $3k+1$. By the Nagell-Lutz theorem over $\mathbb {Q}(\sqrt{-3})$ we have either $y=0$ or $y^2|\Delta$.
Here $\Delta = 4(a+b\sqrt{-3})^3$. So, the options for $$y^2=(a+b\sqrt{-3})^2, 4(a+b\sqrt{-3})^2,4,1$$

Suppose that we have the first case, 
$$y^2=(a+b\sqrt{-3})^2=x^3+(a+b\sqrt{-3})x$$
By applying a norm, we have 
$$N(y)^2=N(x)N(x^2+a+b\sqrt{-3})$$
Therefore, substituting $x=x_1+\sqrt{-3}x_2$, we have 
$$p^2=(x_1^2+3x_2^2)N(x^2+a+\sqrt{-3}b)$$
In this case, we have $(x_1^2+3x_2^2)=p, N(x^2+a+b\sqrt{-3})=p$.
Since a prime can be written in at most one way like $x^2+3y^2$, we have $x_1=a,x_2=b$, in this case we have
$$p=N(x^2+a+b\sqrt{-3})$$
This is the same as
$$p=(x_1^2+3x_2^2)^2+12x_1x_2b+2a(x_1^2-3x_2^2)$$
The above can be written as
$$p=p^2+12x_1x_2b-2ap-12ax_2^2$$
So modulo $p$ we have 
$$x_1x_2b-ax_2^2=0$$
So, $x_2=0$ or $bx_1-ax_2=0$. The only possibility is $bx_1=ax_2$. Hence $x_1=\pm{a},x_2=\pm{b}$ is the only solution. 

Otherwise, we have $x_1^2+3x_2^2=p^2$ and the other quantity
$$1=p^4+12x_1x_2b-2ap^2-12ax_2^2$$
implying that 
$$1=12ax_2(ix_1-x_2) \mod p$$
But, on the other hand, we have 
$$(x_1^2-3x_2^2+a)^2+3(2x_1x_2+b)^2=1$$
Hence, we have
$x_1^2-3x_2^2+a=1, 2x_1x_2+b=0$
From the first,
$x_1^2+3x_2^2-6x_2^2+a=1$
or 
$$p^2-1=6x_2^2-a$$
Also, we have 
$b=-2x_1x_2$
Substituting into the equation $a^2+3b^2=p$ we have
$$12x_1^2x_2^2+(6x_2^2+1-p^2)^2=p$$
Modulo $p$ we have 
$$12x_1^2x_2^2+(6x_2^2+1)^2=0$$
This gives
$$12x_1^2x_2^2+36x_2^2+1+12x_2^2=0$$
$$1+12x_2^2=0$$
modulo $p$. Then we have
$$3x_2^2=pk-1/8$$
Hence, we have 
$$x_1^2+3x_2^2=p^2$$
So, $$x_1^2+pk-1/8=p^2$$
Hence, $$x_1^2=p^2-(\frac{pk-1}{8})$$
Modulo $p$, we have $8x_1^2=1$ so $2$ is a square modulo $p$. So, if we exclude the primes that are congruent to $1, 7$ modulo $24$, then there is no solution.}

